Benchmark of visual and 3D lidar SLAM systems in simulation environment for vineyards

In this work, we present a comparative analysis of the trajectories estimated from various Simultaneous Localization and Mapping (SLAM) systems in a simulation environment for vineyards. Vineyard environment is challenging for SLAM methods, due to visual appearance changes over time, uneven terrain, and repeated visual patterns. For this reason, we created a simulation environment specifically for vineyards to help studying SLAM systems in such a challenging environment. We evaluated the following SLAM systems: LIO-SAM, StaticMapping, ORB-SLAM2, and RTAB-MAP in four different scenarios. The mobile robot used in this study equipped with 2D and 3D lidars, IMU, and RGB-D camera (Kinect v2). The results show good and encouraging performance of RTAB-MAP in such an environment.

==> src/toread.tex <==
%https://introlab.3it.usherbrooke.ca/mediawiki-introlab/images/7/7a/Labbe18JFR_preprint.pdf


%http://www.ladispe.polito.it/corsi/meccatronica/01PCYQW/2012-13/Slides/Reference%20frames%20and%20rotations.pdf
%http://motion.cs.illinois.edu/RoboticSystems/CoordinateTransformations.html
%https://pages.mtu.edu/~shene/COURSES/cs3621/NOTES/geometry/geo-tran.html
%https://pointclouds.org/documentation/tutorials/normal_estimation.html
%https://gtsam.org/tutorials/intro.html

%must read:
%https://ieeexplore.ieee.org/document/1267047
%https://ieeexplore.ieee.org/document/910572

